Weak-Driven Learning: How Weak Agents make Strong Agents Stronger

As post-training optimization becomes central to improving large language models, we observe a persistent saturation bottleneck: once models grow highly confident, further training yields diminishing returns. While existing methods continue to reinforce target predictions, we find that informative supervision signals remain latent in models' own historical weak states. Motivated by this observation, we propose WMSS (Weak Agents Can Make Strong Agents Stronger), a post-training paradigm that leverages weak checkpoints to guide continued optimization. By identifying recoverable learning gaps via entropy dynamics and reinforcing them through compensatory learning, WMSS enables strong agents to improve beyond conventional post-training saturation. Experiments on mathematical reasoning and code generation datasets show that agents trained with our approach achieve effective performance improvements, while incurring zero additional inference cost.

==> content/2_related_work_old.tex <==
% \section{Related Work}

% \subsection{Post-training Optimization and Data Selection}
% As scaling laws saturate~\cite{kaplan2020scaling, hoffmann2022training}, the focus has shifted to post-training strategies. However, treating all data equally often leads to optimization stagnation. To address this, Curriculum Learning~\cite{bengio2009curriculum} proposes organizing data from easy to hard. Beyond static ordering, dynamic reweighting strategies such as \textbf{Focal Loss}~\cite{lin2017focal} and \textbf{Online Hard Example Mining (OHEM)}~\cite{shrivastava2016training} modify the objective function to up-weight samples with high instantaneous loss, forcing the model to focus on difficult instances. In the context of LLMs, recent works also employ perplexity-based filtering or complexity scoring~\cite{chen2023alpagasus} to select high-quality instruction data.

% However, these approaches suffer from significant limitations. Relying on \textbf{instantaneous loss or perplexity} makes them highly susceptible to stochastic optimization noise: a spike in loss often indicates data noise or outliers rather than learnable difficulty, leading to instability or overfitting~\cite{katharopoulos2018not}. Furthermore, static reweighting fails to adapt to the model's evolving competence.
% Our work advances this by introducing \textbf{Entropy-Guided Battlefield Selection}. By analyzing the \emph{longitudinal entropy trajectory} rather than instantaneous snapshots, we decouple intrinsic difficulty from transient noise. We treat high entropy as a robust signal of the ``zone of proximal development,'' specifically targeting the saddle points where the model's historical self struggles, ensuring optimization effort is invested where it yields the highest marginal return.

% \subsection{From Knowledge Distillation to Compensatory Learning}
% Knowledge Distillation (KD)~\cite{hinton2015distilling} and its LLM variants like Evol-Instruct~\cite{xu2023wizardlm} rely on a core assumption: the student should \emph{imitate} the teacher. Even in Weak-to-Strong Generalization~\cite{burns2023weak}, the goal remains to extract latent knowledge from a supervisor. However, self-imitation creates a feedback loop that leads to \emph{model collapse} or confirmation bias~\cite{shumailov2023curse, alemohammad2023selfconsuminggenerativemodelsmad}.

% \modelname fundamentally diverges from this imitation paradigm. We propose \textbf{Compensatory Learning}, where the historical checkpoint serves not as a teacher to be mimicked, but as a \emph{sacrificial anchor} to be overcome. By forcing the primary model to compensate for the decaying logits of its historical self, we transform the risk of model collapse into a mechanism for \emph{residual error correction}, effectively utilizing the historical model's failure modes to define the direction of improvement.

% \subsection{Multi-Model Dynamics: Competition vs. Collaboration}
% Multi-model systems, such as ensembles and boosting methods~\cite{chen2025llmboost, zou2025transformer}, improve performance by aggregating diverse predictors. However, they incur prohibitive inference costs. More efficient approaches like Mutual Learning (DML)~\cite{zhang2018deep, anil2018large} reduce costs but suffer from \emph{mean-seeking} behavior~\cite{zhu2018knowledge}, where symmetric peers converge to a safe average rather than exploring superior local optima.

% Our work is distinct in its utilization of \textbf{Gradient Monopoly} and \textbf{Gradient Starvation}~\cite{pezeshki2021gradientstarvationlearningproclivity}. While prior work in multi-task learning views \emph{gradient conflict} as a pathology to be cured (e.g., Gradient Surgery~\cite{yu2020gradientsurgerymultitasklearning}), we harness it as a driving force. By placing the primary model in a zero-sum logit fusion with its history, we induce a dynamic where the stronger model monopolizes the gradient signal. This allows \modelname to achieve the performance benefits of competitive dynamics without the inference overhead of ensembles, as the collapsed auxiliary branch is discarded after training.

\section{Related Work}
\label{sec:related_work}

\subsection{Supervised Fine-Tuning and Optimization Saturation} Supervised Fine-Tuning (SFT) is the dominant paradigm for aligning Large Language Models~\cite{ouyang2022training, touvron2023llama}. However, the "Superficial Alignment Hypothesis" proposed by \cite{zhou2024lima} suggests that SFT primarily adapts interaction styles rather than injecting new knowledge. Consequently, SFT often encounters a saturation bottleneck in reasoning-intensive tasks. For instance, \cite{shao2024deepseekmath} demonstrate that on mathematical benchmarks, standard SFT quickly plateaus, necessitating Reinforcement Learning (RL) to further optimize the decision boundary.

To break this bottleneck without the complexity of RL, recent works have explored Iterative Self-Improvement . notably, SPIN~\cite{chen2024self} utilizes the model's previous iteration to generate negative samples, constructing a self-play mechanism within the SFT format. similarly, \cite{burns2023weak} explore Weak-to-Strong Generalization , showing that stronger models can infer latent ground truth even from weak supervisors.

\modelname{} unifies these insights. Unlike SPIN which requires expensive generation of new synthetic data, we leverage the historical weak checkpoints directly. By analyzing the entropy shift between the weak and strong states, we identify recoverable learning gaps and reignite gradient flow, effectively extending the efficacy of SFT beyond its conventional saturation point.

\subsection{Dynamic Data Selection and Curriculum Learning} 
Selecting the right data is pivotal for efficient post-training~\cite{albalak2024survey}. Traditional Curriculum Learning~\cite{bengio2009curriculum} or filtering methods (eg, AlpaGasus~\cite{chen2023alpagasus}) typically rely on static snapshots of difficulty, such as current loss or perplexity. However, static metrics are ambiguous: a high-loss sample could be a valuable hard instance or simply noise~\cite{katharopoulos2018not}. Recent research shifts towards Training Dynamics , tracking model behavior over time to distinguish learnable samples from outliers~\cite{swayamdipta2020dataset}. \modelname{} advances this by introducing Entropy Dynamics . Instead of static uncertainty, we measure the relative entropy shift ($\Delta H$) between weak and strong states. This allows us to specifically target catastrophic forgetting —recoverable learning gaps—rather than irreducible data noise.

\subsection{Weak-to-Strong Generalization and Semantic Regularization} Improving strong models usually relies on stronger supervisors (eg, GPT-4 distillation). However, as models approach the frontier, such supervision becomes scarce. This has sparked interest in Weak-to-Strong Generalization ~\cite{burns2023weak}, exploring how weak signals can elicit strong latent capabilities. Simultaneously, regularization techniques like NEFTune ~\cite{jain2023neftunenoisyembeddingsimprove} demonstrate that injecting noise into embeddings can prevent overfitting and improve robustness.

\modelname bridges these paradigms via Compensatory Learning . First, unlike standard Knowledge Distillation~\cite{hinton2015distilling} which encourages imitation of a teacher, we use the historical weak agent as a contrastive reference . Second, unlike NEFTune which injects random noise, we inject plausible but incorrect tokens —specifically, the logits of the weak model's errors. This acts as a structured regularizer that selectively amplifies gradients on the model's historical confusion boundaries. By suppressing plausible distractors from the past, we force the strong agent to refine its decision boundary beyond the saturation point of standard SFT.

==> content/3_methods_old.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

We consider a language model $\mathcal{M}_{\theta}$ that maps an input sequence $x$ to a next-token distribution over vocabulary $\mathcal{V}$. Let $z_t \in \mathbb{R}^{|\mathcal{V}|}$ denote the output \textbf{logits} at step $t$. The probability of a token is given by the softmax function $P(y|x) = \text{Softmax}(z_t)$.

In standard Supervised Fine-Tuning (SFT), we minimize the negative log-likelihood over a dataset $\mathcal{D}$:
\begin{equation}
    \mathcal{L}_{\text{SFT}}(\theta) = - \mathbb{E}_{(x,y) \sim \mathcal{D}} \left[ \log P(y | x; \theta) \right]
\end{equation}
To measure model uncertainty and stagnation, we monitor the \textbf{predictive entropy} $H(P) = - \sum P(v) \log P(v)$.
Crucially, for Cross-Entropy loss, the gradient magnitude regarding a negative token $k$ is proportional to its probability: $|\nabla_{z[k]} \mathcal{L}| = P(k)$. Our method exploits this property: by artificially inflating $P(k)$ via logit injection, we amplify the learning signal for hard negatives.

\section{Methodology}
\label{sec:methodology}

% \subsection{Make weak model}
\subsection{Weak-Reference Initialization}
In the \modelname framework, the \textbf{weak} (\textit{Confuser}) model (denoted as $\mathcal{M}_{t-1}$ or $\mathcal{M}_{\text{ref}}$) acts as the repository of historical knowledge and the source of structured priors.

% \paragraph{Establishing the Semantic Guidance Prior.} 
% The process begins in Phase 1 (Initialization), where a base model $\mathcal{M}_0$ undergoes standard SFT to produce the initial baseline $\mathcal{M}_1$. For any subsequent iteration $t$, the logits generated by the previous state $\mathcal{M}_{t-1}$ are defined as the \textbf{Semantic Guidance Prior} ($z_{\text{ref}}$). 
\paragraph{Weak-Checkpoint Semantic Guidance Prior.} 
The process begins in Phase 1 (Initialization), where a base model $\mathcal{M}_0$ undergoes standard SFT to produce the initial baseline $\mathcal{M}_1$. We intentionally treat this SFT-only model as the \emph{weak} (Confuser) reference: it captures the core decision boundary but typically saturates on hard reasoning samples. For any subsequent iteration $t$, the logits generated by the previous state $\mathcal{M}_{t-1}$ are defined as the \textbf{Semantic Guidance Prior} ($z_{\text{ref}}$). 



Unlike isotropic random noise, this prior captures the model's historical "soft" decision boundaries. High-value logits in $z_{\text{ref}}$ correspond to plausible but incorrect distractors ("hard negatives"). This ensures the noise injected during training is targeted specifically at the model's historical blind spots, providing a structured map for the next generation of evolution.



% \subsection{Make strong model}
% The \textbf{strong model} ($\mathcal{M}_t$) represents the current active learner. While it possesses superior overall performance, its strength is non-uniform, exhibiting localized learning stagnation or regression that requires diagnostic identification.
\subsection{Curriculum-Enhanced Strong Model}
The \textbf{strong} (\textit{Learner}) model $\mathcal{M}_t$ represents the current active learner, obtained by continuing SFT on an entropy-guided curriculum. This curriculum-weighted SFT yields a learner that is consistently stronger than the plain SFT baseline, but still exhibits localized learning stagnation or regression that requires diagnostic identification.


\paragraph{Mapping Entropy Dynamics.} 
To distinguish between irreducible data noise and learnable concepts, we model the uncertainty shift between the weak (Confuser) and strong (Learner) states. Let $\Delta H_i = H(x_i; \theta_t) - H(x_i; \theta_{t-1})$ denote the entropy shift. 

\paragraph{Curriculum Construction via Learning Stagnation.}
To construct a robust training distribution, we formulate the sampling probability $p_i$ as a weighted mixture of three distinct learning signals derived from these entropy dynamics:
\vspace{-2pt}
\begin{equation}
    \label{eq:sampling_prob}
    \begin{split}
        p_i &= \underbrace{\alpha \cdot \frac{H(x_i; \theta_{t-1})}{Z_1}}_{\text{Base Difficulty}} 
             + \underbrace{\beta \cdot \frac{|\Delta H_i| \cdot \mathbb{I}(\Delta H_i < 0)}{Z_2}}_{\text{Consolidation}} \\ 
             & + \underbrace{\gamma \cdot \frac{\Delta H_i \cdot \mathbb{I}(\Delta H_i > 0)}{Z_3}}_{\text{Regression Repair}}
    \end{split}
\end{equation}

where $\mathbb{I}(\cdot)$ is the indicator function and $Z_{1,2,3}$ are normalization constants. The hyperparameters $\beta$ and $\gamma$ address two critical learning states:

\begin{itemize}
    \item \textbf{Base Difficulty Assessment ($\alpha$ term):} 
    This term captures the intrinsic difficulty of a sample based on the weak checkpoint.
    We use the predictive entropy $H(x_i; \theta_{t-1})$ as a measure of how uncertain the earlier model was on $x_i$,
    indicating concepts that were historically hard to resolve.
    By up-weighting samples with higher historical entropy, this component ensures that inherently difficult examples
    are consistently emphasized during training, providing a stable baseline signal independent of short-term entropy shifts.

    \item \textbf{Retention Reinforcement ($\beta$ term, $\Delta H < 0$):} 
    This targets samples where uncertainty has decreased. A negative shift implies effective acquisition; however, if the drop is large, the knowledge may be fragile. By weighting these samples, we perform \emph{consolidation}, ensuring "fast-learned" concepts are etched into long-term memory.
    
    \item \textbf{Regression Repair ($\gamma$ term, $\Delta H > 0$):} 
    Focusing on samples where uncertainty has increased. Crucially, a positive shift implies that the previous weak (Confuser) model $\mathcal{M}_{t-1}$ handled the sample better than the current Learner $\mathcal{M}_t$. This confirms the sample is \textbf{valid and learnable}, ruling out irreducible noise. Therefore, a large positive $\Delta H$ signifies \textbf{Catastrophic Forgetting}. We amplify these samples to forcefully "repair" the learner's regression and retrieve the lost decision boundary.
\end{itemize}

This curriculum-trained model $\mathcal{M}_t$ serves as the Learner model in the next stage, where it is further improved by joint training with the weak (Confuser) reference.



% The core of \modelname lies in the \emph{Residual Evolution} paradigm, where the "weak" model's residuals are leveraged to push the "strong" model into a \textbf{stronger} state $\mathcal{M}_{t+1}$ via Gradient Amplification.


\subsection{Joint Training with Weak Reference to Strengthen the Strong Model}
The core of \modelname lies in the joint Evolution paradigm: given a weak reference $\mathcal{M}_{\mathrm{weak}}$ and a curriculum-trained strong model $\mathcal{M}_{\mathrm{strong}}$, we leverage the weak agent as the reference to push the strong agent into a \textbf{stronger} state $\mathcal{M}_{t+1}$. 
This joint-training step is the explicit \emph{Confuser + Learner $\rightarrow$ stronger Learner} step of our narrative.


\paragraph{Constructing the Residual Guidance Map.} 
During the \emph{Compensatory Joint Training} phase, we linearly interpolate the Learner's logits $z_{\theta}$ with the \textbf{Semantic Guidance Prior} $z_{\text{ref}}$ to construct a \textbf{Residual Guidance Map}:
\begin{equation}
    \label{eq:logit_mix}
    z_{\text{mix}} = \lambda \cdot z_{\theta} + (1-\lambda) \cdot z_{\text{ref}}
\end{equation}
where $\lambda$ controls the mixing intensity. This mechanism prevents gradient vanishing on "distractor" tokens by reinvigorating the optimization landscape with historical confusion.

\paragraph{Gradient Amplification Dynamics.} 
The interaction between the \textbf{Residual Guidance Map} and the Cross-Entropy loss triggers a targeted amplification effect. For a distractor token $k$, the \textbf{Semantic Guidance Prior} $z_{\text{ref}}$ contributes a \textbf{guidance peak}, artificially inflating the combined probability $P_{\text{mix}}(k)$ in the mixed logit space. Given that the gradient magnitude for a negative class is proportional to its predicted probability ($|\nabla_{z[k]} \mathcal{L}| \propto P(k)$), this inflation triggers \textbf{Gradient Amplification}. The optimizer perceives a magnified error on these specific historical blind spots. To minimize this amplified penalty, the Learner $z_{\theta}$ is mathematically compelled to \textbf{"over-correct,"} learning significantly lower logits to counteract the injected prior. This effectively converts historical confusion into a robust supervision signal, forcing the Learner to refine its decision boundary exactly where it was previously ambiguous.



\begin{algorithm}[t]
  \caption{\modelname: Iterative Compensatory Evolution}
  \label{alg:training_pipeline}
  \begin{algorithmic}[1]
    \REQUIRE Dataset $\mathcal{D}$, Base Model $\mathcal{M}_0$
    \REQUIRE Iterations $K$, Hyperparams $\alpha, \beta, \gamma, \lambda$
    \STATE \textbf{Phase 1: Initialization}
    \STATE $\mathcal{M}_1 \leftarrow \text{Train}(\mathcal{M}_0, \mathcal{D}, \mathcal{L}_{\text{SFT}})$ \COMMENT{Establish initial weak (Confuser) reference}
    \STATE \textbf{Phase 2: Iterative Evolution Loop}
    \FOR{$t = 1$ to $K$}
        \STATE \textit{// Step A: Curriculum Assessment}
        \STATE $\Delta \mathbf{H} \leftarrow \mathbf{H}(\mathcal{M}_t) - \mathbf{H}(\mathcal{M}_{t-1})$
        \STATE Calculate $\mathbf{p}$ via Eq.~\ref{eq:sampling_prob} using $\Delta \mathbf{H}$ and $\mathbf{H}(\mathcal{M}_{t-1})$
        \STATE $\mathcal{D}_{\text{active}} \leftarrow \text{WeightedSample}(\mathcal{D}, \mathbf{p})$
        
        \STATE \textit{// Step B: Residual Guidance Training}
        \STATE Initialize $\mathcal{M}_{\theta} \leftarrow \mathcal{M}_{t}$
        \FOR{batch $(x, y) \in \mathcal{D}_{\text{active}}$}
            \STATE $z_{\text{ref}} \leftarrow \text{Forward}(\mathcal{M}_{t-1}, x)$ \COMMENT{Retrieve Semantic Guidance Prior}
            \STATE $z_{\text{mix}} \leftarrow \lambda z_{\theta} + (1-\lambda)z_{\text{ref}}$ \COMMENT{Apply Residual Guidance Map}
            \STATE Update $\mathcal{M}_{\theta}$ via $\nabla \text{CE}(z_{\text{mix}}, y)$ \COMMENT{Gradient Amplification}
        \ENDFOR
        \STATE $\mathcal{M}_{t+1} \leftarrow \mathcal{M}_{\theta}$
    \ENDFOR
    \STATE \textbf{return} $\mathcal{M}_{K+1}$
  \end{algorithmic}
\end{algorithm}
\vspace{-5pt}




% \subsection{Curriculum Construction via Entropy Dynamics}
% \label{sec:entropy_signal}

% Standard curriculum learning often relies on static difficulty metrics. In contrast, we model the \emph{dynamics} of uncertainty to distinguish between irreducible noise and learnable concepts. We introduce a \textbf{Learning Stagnation \modelname} derived from the entropy shift between the weak model $\mathcal{M}_{t-1}$ and a strong model $\mathcal{M}_t$.

% \paragraph{Sampling Probability Construction.}
% To construct a robust training distribution, we formulate the sampling probability $p_i$ as a weighted mixture of three distinct learning signals derived from entropy dynamics. Let $\Delta H_i = H(x_i; \theta_t) - H(x_i; \theta_{t-1})$ denote the entropy shift. The final sampling probability is defined as:

% \begin{equation}
%     \label{eq:sampling_prob}
%     \begin{split}
%         p_i &= \underbrace{\alpha \cdot \frac{H(x_i; \theta_{t-1})}{Z_1}}_{\text{Base Difficulty}} 
%              + \underbrace{\beta \cdot \frac{|\Delta H_i| \cdot \mathbb{I}(\Delta H_i < 0)}{Z_2}}_{\text{Consolidation}} \\ 
%              & + \underbrace{\gamma \cdot \frac{\Delta H_i \cdot \mathbb{I}(\Delta H_i > 0)}{Z_3}}_{\text{Regression Repair}}
%     \end{split}
% \end{equation}

% where $\mathbb{I}(\cdot)$ is the indicator function. The hyperparameters $\alpha, \beta, \gamma$ balance three curriculum objectives:

% \begin{itemize}
%     \item \textbf{Base Difficulty Assessment ($\alpha$ term):} 
%     This term anchors the curriculum on intrinsic complexity using the historical uncertainty $H_{t-1}$. It ensures basic coverage of challenging concepts regardless of training dynamics.

%     \item \textbf{Retention Reinforcement ($\beta$ term, $\Delta H < 0$):} 
%     Targeting samples where uncertainty has decreased. A negative shift implies effective acquisition. However, if the drop is small, the learning is stable; if the drop is large, the knowledge might be fragile. By weighting these samples, we perform \emph{consolidation}, ensuring "fast-learned" concepts are etched into long-term memory.

%     \item \textbf{Regression Repair ($\gamma$ term, $\Delta H > 0$):} 
%     Focusing on samples where uncertainty has increased. 
%     Crucially, a positive shift ($\Delta H > 0$) implies that the previous model $\mathcal{M}_{t-1}$ handled this sample better than the current $\mathcal{M}_t$. This confirms the sample is \textbf{valid and learnable}, ruling out irreducible data noise. 
%     Therefore, a large positive $\Delta H$ signifies \textbf{Catastrophic Forgetting} rather than data outliers. We proportionally amplify these samples to forcefully "repair" the model's regression and retrieve the lost decision boundary.
% \end{itemize}

% \begin{algorithm}[t]
%   \caption{\modelname: Iterative Compensatory Evolution}
%   \label{alg:SONAR_iterative}
%   \begin{algorithmic}[1]
%     \REQUIRE Dataset $\mathcal{D}$, Base Model $\mathcal{M}_0$
%     \REQUIRE Iterations $K$, Hyperparams $\alpha, \beta, \gamma$ (Curriculum Weights), $\lambda$ (Mixing Coeff)
    
%     \STATE \textbf{Phase 1: Initialization (Reference Establishment)}
%     \STATE $\mathcal{M}_1 \leftarrow \text{Train}(\mathcal{M}_0, \mathcal{D}, \mathcal{L}_{\text{SFT}})$ \COMMENT{Establish initial baseline}
    
%     \STATE \textbf{Phase 2: Iterative Evolution Loop}
%     \FOR{$t = 1$ to $K$}
%         \STATE \textit{// Step A: Curriculum Probability Assessment}
%         \STATE Let $\mathcal{M}_{\text{ref}} \leftarrow \mathcal{M}_{t-1}$ \COMMENT{Historical Reference}
%         \STATE Let $\mathcal{M}_{\text{cur}} \leftarrow \mathcal{M}_{t}$ \COMMENT{Current Snapshot}
        
%         \STATE \textit{// 1. Compute Entropy Dynamics (Vectorized)}
%         \STATE $\mathbf{H}_{\text{ref}} \leftarrow \{ H(\mathcal{M}_{\text{ref}}, x) \mid x \in \mathcal{D} \}$
%         \STATE $\mathbf{H}_{\text{cur}} \leftarrow \{ H(\mathcal{M}_{\text{cur}}, x) \mid x \in \mathcal{D} \}$
%         \STATE $\Delta \mathbf{H} \leftarrow \mathbf{H}_{\text{cur}} - \mathbf{H}_{\text{ref}}$
        
%         \STATE \textit{// 2. Construct Sampling Distribution}
%         \STATE Calculate probability vector $\mathbf{p}$ via Eq.~ref{eq:sampling_prob} using $\Delta \mathbf{H}$ and $\mathbf{H}_{\text{ref}}$
        
%         \STATE \textit{// 3. Selection}
%         \STATE $\mathcal{D}_{\text{active}} \leftarrow \text{WeightedSample}(\mathcal{D}, \mathbf{p})$ \COMMENT{Curriculum-based Sampling}
        
%         \STATE \textit{// Step B: Compensatory Joint Training}
%         \STATE Initialize Active Learner $\mathcal{M}_{\theta} \leftarrow \mathcal{M}_{t}$ \COMMENT{Will become $\mathcal{M}_{t+1}$}
%         \FOR{batch $(x, y) \in \mathcal{D}_{\text{active}}$}
%             \STATE $z_{\text{ref}} \leftarrow \text{Forward}(\mathcal{M}_{\text{ref}}, x)$ \COMMENT{Get Semantic Noise Map}
%             \STATE $z_{\theta} \leftarrow \text{Forward}(\mathcal{M}_{\theta}, x)$ \COMMENT{Get Active Logits}
            
%             \STATE \textit{// Targeted Noise Injection (Eq.~ref{eq:logit_mix})}
%             \STATE $z_{\text{mix}} \leftarrow \lambda \cdot z_{\theta} + (1-\lambda) \cdot z_{\text{ref}}$
            
%             \STATE Update $\mathcal{M}_{\theta}$ via $\nabla \text{CE}(z_{\text{mix}}, y)$ \COMMENT{Gradient Amplification}
%         \ENDFOR
%         \STATE $\mathcal{M}_{t+1} \leftarrow \mathcal{M}_{\theta}$
%     \ENDFOR
    
%     \STATE \textbf{return} $\mathcal{M}_{K+1}$
%   \end{algorithmic}
% \end{algorithm}

% \subsection{Gradient Amplification via Semantic Noise Injection}
% \label{sec:SONAR_training}

% Standard SFT optimization often stagnates as gradients on "distractor" tokens vanish once the target probability dominates. To counteract this, we introduce a \textbf{Compensatory Noise Injection} mechanism that leverages historical confusion to reinvigorate training.

% \paragraph{Targeted Logit Integration.}
% Instead of introducing indiscriminate random perturbations, we utilize the historical reference model $\mathcal{M}_{\text{ref}}$ (typically the previous snapshot $\mathcal{M}_{t-1}$) as a source of structured semantic noise. We perform a linear interpolation of logits during the forward pass:
% \begin{equation}
%     \label{eq:logit_mix}
%     z_{\text{mix}} = \lambda \cdot z_{\theta} + (1-\lambda) \cdot z_{\text{ref}}
% \end{equation}
% where $z_{\theta}$ represents the active learner and $(1-\lambda)$ controls the noise magnitude. Unlike isotropic random noise, $z_{\text{ref}}$ acts as a \textbf{semantic map}, where high values correspond to plausible but incorrect distractors ("hard negatives"). This ensures the noise is targeted specifically at the model's historical blind spots.

% \paragraph{Gradient Amplification Dynamics.}
% The core innovation lies in the interaction between this injected noise and the Cross-Entropy loss. For a distractor token $k$, the reference model contributes a high "noise spike" ($z_{\text{ref}}[k]$), artificially inflating the combined probability $P_{\text{mix}}(k)$.
% Given that the gradient magnitude for a negative class is proportional to its probability ($|\nabla_{z[k]} \mathcal{L}| \propto P(k)$)~\cite{lin2018focallossdenseobject}, this inflation triggers \textbf{Gradient Amplification}. The optimizer perceives a magnified error on these specific tokens. To minimize this amplified penalty, the active learner $z_{\theta}$ is mathematically compelled to "over-correct," learning significantly lower logits to counteract the injected noise. This effectively converts historical confusion into a robust supervision signal, forcing the model to refine its decision boundary exactly where it is most ambiguous.




% \vspace{-10pt}
\subsection{Training Pipeline}
The comprehensive workflow of \modelname is detailed in Algorithm~\ref{alg:training_pipeline}. The process commences with \textbf{Phase 1 (Initialization)}, where a standard SFT model $\mathcal{M}_1$ is derived from the base model $\mathcal{M}_0$ to establish a foundational decision boundary and provide the initial \textbf{Semantic Guidance Prior} (the Confuser anchor) for the subsequent evolutionary loop.

% Subsequently, \textbf{Phase 2} executes an iterative evolutionary loop (Lines 4--19). Unlike static training, this phase dynamically updates the curriculum in each iteration $t$. First, the algorithm evaluates the \textit{entropy dynamics} between the previous snapshot ($\mathcal{M}_{t-1}$) and the current state ($\mathcal{M}_{t}$) to identify stagnation, producing a curriculum-weighted dataset $\mathcal{D}_{\text{active}}$. 
% Then, during the training of the candidate $\mathcal{M}_{t+1}$, the previous model $\mathcal{M}_{t-1}$ serves as a \textbf{historical "noise generator."} By linearly injecting the historical logits $z_{\text{ref}}$ into the current forward pass, the active learner is mathematically compelled to over-correct against its past errors. This mechanism effectively converts historical confusion into a gradient amplification signal, robustifying the model against distractor tokens.

Subsequently, \textbf{Phase 2} executes an iterative evolutionary loop (Lines 4--19). Conceptually, each iteration contains two substeps: (i) curriculum-weighted SFT that yields the current strong (Learner) snapshot $\mathcal{M}_{t}$, and (ii) joint training that combines the weak (Confuser) snapshot $\mathcal{M}_{t-1}$ with the Learner $\mathcal{M}_{t}$ to produce a stronger $\mathcal{M}_{t+1}$. In practice, we implement this as a unified loop that updates the curriculum each iteration. First, the algorithm evaluates the \textit{entropy dynamics} between the Confuser snapshot ($\mathcal{M}_{t-1}$) and the Learner state ($\mathcal{M}_{t}$) to identify stagnation, producing a curriculum-weighted dataset $\mathcal{D}_{\text{active}}$. The subsequent joint-training step then mixes logits as in Eq.~\ref{eq:logit_mix}, allowing the Learner to suppress Confuser-revealed distractors and continue strengthening beyond saturation.


\vspace{-10pt}
\section{Theoretical Analysis: Gradient Amplification and Margin Expansion}
\label{sec:theoretical_analysis}

In this section, we provide two complementary theoretical views. First, we formalize why \textbf{joint logit mixing amplifies negative-token gradients}, yielding a principled advantage over standard SFT. Second, we retain the original margin-expansion analysis as a complementary lens on how compensatory pressure reshapes decision boundaries.
\vspace{-10pt}
\subsection{Why Joint Training Amplifies Hard-Negative Gradients}
\label{sec:grad_amplification_main}
Consider two models (Confuser/weak $m_1$, Learner/strong $m_2$) with logits $z_1, z_2 \in \mathbb{R}^C$, and the mixed logits
\begin{equation}
    z_{\text{mix}} = (1-\lambda) z_1 + \lambda z_2, \quad \lambda \in (0,1).
    \label{eq:main_mix}
\end{equation}
Let $y$ denote the target index, $e_y$ the one-hot vector, and $p(z)=\text{Softmax}(z)$. The cross-entropy gradient on fused logits is
\begin{equation}
    g_{\text{mix}} = \nabla_{z_{\text{mix}}}\mathcal{L} = p(z_{\text{mix}}) - e_y,
    \label{eq:main_grad_mix}
\end{equation}
while standard SFT on the Learner model gives $g_{\text{sft}} = p(z_2) - e_y$.

\paragraph{Margins and hard negatives.}
Define the target margin for any negative token $k \neq y$ as
\begin{equation}
    m_k(z) = z_y - z_k.
    \label{eq:main_margin_def}
\end{equation}
The Confuser model encodes confusion, so we define the hard-negative set
\begin{equation}
    \mathcal{H} = \{ k \neq y : m_k(z_1) < m_k(z_2) \}.
    \label{eq:main_hard_set}
\end{equation}
The mixed margin is a convex combination:
\begin{equation}
    m_k(z_{\text{mix}}) = (1-\lambda)m_k(z_1) + \lambda m_k(z_2).
    \label{eq:main_margin_mix}
\end{equation}

\begin{theorem}[Total negative-mass increase under uniform margin shrinkage]
If $m_k(z_1) \le m_k(z_2)$ for all $k \neq y$, then
\begin{align}
    p(z_{\text{mix}})_y &\le p(z_2)_y, \nonumber\\
    \sum_{k \neq y} p(z_{\text{mix}})_k &\ge \sum_{k \neq y} p(z_2)_k.
    \label{eq:main_total_neg_mass}
\end{align}
\end{theorem}
\begin{proof}[Proof sketch]
Using $p(z)_k/p(z)_y = \exp(-m_k(z))$, margin shrinkage implies $\exp(-m_k(z_{\text{mix}})) \ge \exp(-m_k(z_2))$ for all $k \neq y$, increasing the denominator of $p(z)_y$ and thus the total negative mass. A full proof is in Appendix~\ref{sec:appendix_grad_amp}.
\end{proof}

\begin{corollary}[Per-token amplification on hard negatives]
For any $k \in \mathcal{H}$, the mixed negative gradient satisfies
\begin{align}
    p(z_{\text{mix}})_k &\ge p(z_2)_k \quad \text{whenever} \nonumber\\
    \frac{p(z_{\text{mix}})_y}{p(z_2)_y}
    &\ge \exp\!\left(-(1-\lambda)\Delta m_k\right),
    \label{eq:main_amp_condition}
\end{align}
where $\Delta m_k = m_k(z_2)-m_k(z_1)>0$.
\end{corollary}
\begin{proof}[Proof sketch]
Express $p_k$ via log-odds, substitute the mixed margin, and rearrange the ratio condition. See Appendix~\ref{sec:appendix_grad_amp} for the full derivation.
\end{proof}

\begin{proposition}[Logit updates emphasize negative suppression]
Under joint training, for model $i \in \{1,2\}$ with scale $s_1=1-\lambda$, $s_2=\lambda$,
\begin{align}
    \Delta z_{i,k} &\approx -\eta s_i\, p(z_{\text{mix}})_k \quad (k \neq y), \nonumber\\
    \Delta z_{i,y} &\approx \eta s_i\, (1-p(z_{\text{mix}})_y).
    \label{eq:main_update}
\end{align}
Thus any increase in $p(z_{\text{mix}})_k$ directly amplifies suppression of hard negatives, while a decrease in $p(z_{\text{mix}})_y$ strengthens the upward push on the target logit.
\end{proposition}
\begin{proof}[Proof sketch]
This follows from $\nabla_{z_i}\mathcal{L}=s_i(p(z_{\text{mix}})-e_y)$ and a first-order update $\Delta z_i \approx -\eta \nabla_{z_i}\mathcal{L}$. See Appendix~\ref{sec:appendix_grad_amp}.
\end{proof}

\paragraph{Interpretation.}
These results formalize the key advantage over SFT: mixing logits redistributes probability mass toward hard negatives, which \emph{increases their gradients} and drives stronger suppression of incorrect tokens. This mechanism aligns with our empirical logit statistics (noise floor reduction and heavier tails) and provides a causal explanation for improved accuracy on hard tasks.

\paragraph{Mechanistic interpretation (summary).}

Beyond local gradients, joint training induces a three-stage dynamic: early gradient-share dominance of the Learner model (amplified by Confuser hard negatives), gradient shielding, and null-space drift. We include a formal analysis in Appendix~\ref{sec:appendix_joint_theory}; in short, the Confuser model exposes confusion regions early on, the Learner model takes the dominant update signal as it stabilizes, and mean-shift directions remain unconstrained. This interpretation complements the gradient-amplification view and explains the observed logit mean shifts.


In this section, we also provide a complementary margin-expansion analysis under a linearized MSE regime, which offers an alternative perspective on how compensatory pressure reshapes decision boundaries.


% \subsection{Problem Formulation}

% Let $(x, y)$ be a training sample, where $y \in \mathbb{R}$ represents the scalar target logit for the correct class (e.g., a high confidence value $y > 0$). We define the training system as:
% \begin{itemize}
%     \item \textbf{Primary Model (Trainable):} $f(x; \theta)$, parameterized by $\theta$.
%     \item \textbf{Auxiliary Anchor (Frozen):} $f_{\text{anc}}(x)$, derived from a historical checkpoint and kept fixed during this phase.
% \end{itemize}

% The training objective minimizes the loss of the fused prediction with a mixing coefficient $\lambda \in (0, 1)$:
% \begin{equation}
%     \label{eq:SONAR_loss}
%     \mathcal{L}(\theta) = \frac{1}{2} \mathbb{E}_{(x,y)} \left[ \left( \lambda f(x; \theta) + (1-\lambda) f_{\text{anc}}(x) - y \right)^2 \right]
% \end{equation}

% \subsection{Adaptive Margin Expansion}

% To understand the effective optimization target imposed on the primary model, we analyze the stationary condition of the loss function. Setting the gradient $\nabla_\theta \mathcal{L} = 0$, the optimal state $f(x; \theta^*)$ must satisfy:
% \begin{equation}
%     \lambda f(x; \theta^*) + (1-\lambda) f_{\text{anc}}(x) = y
% \end{equation}
% Solving for the primary model's output $f(x; \theta^*)$:
% \begin{equation}
%     \label{eq:effective_target}
%     f(x; \theta^*) = \frac{y - (1-\lambda) f_{\text{anc}}(x)}{\lambda} = y + \frac{1-\lambda}{\lambda} \underbrace{(y - f_{\text{anc}}(x))}_{\text{Historical Residual}}
% \end{equation}
% Equation~\ref{eq:effective_target} reveals that the primary model is not simply learning the ground truth $y$. Instead, it learns an \textbf{augmented target} comprising the original label plus a scaled version of the historical error. This confirms that \modelname performs \emph{residual evolution}.

% We now formally show that this mechanism is \textbf{adaptive}: it imposes a heavy ``resistance load'' on hard samples while remaining neutral on mastered data.

% \begin{theorem}[\textbf{Adaptive Margin Expansion}]
%     \label{thm:adaptive_margin}
%     Assuming an equiprobable mixing strategy ($\lambda = 0.5$), the convergence target for the primary model adapts to the historical difficulty of the sample:
    
%     \begin{enumerate}
%         \item \textbf{Regime I: Easy Samples (Stability).} 
%         If the historical anchor is already confident ($f_{\text{anc}}(x) \approx y$), then the effective target becomes:
%         \begin{equation}
%             f(x; \theta^*) \approx y + (y - y) = y
%         \end{equation}
%         In this regime, the auxiliary branch provides no resistance, and the training reduces to standard Supervised Fine-Tuning (SFT), preserving stability on mastered knowledge.
        
%         \item \textbf{Regime II: Hard Samples (Expansion).} 
%         If the sample corresponds to a saddle point where the historical anchor exhibits high entropy or collapse ($f_{\text{anc}}(x) \approx 0$), the effective target becomes:
%         \begin{equation}
%             f(x; \theta^*) \approx y + (y - 0) = 2y
%         \end{equation}
%         Here, the frozen anchor acts as a dead weight. To satisfy the objective, the primary model is forced to generate logits with \textbf{double the magnitude}, effectively expanding the classification margin by a factor of $1/\lambda$.
%     \end{enumerate}
% \end{theorem}

% \subsection{Interpretation as Resistance Training}

% The phenomenon described in Theorem~ref{thm:adaptive_margin} provides a rigorous mathematical justification for the ``resistance training'' metaphor. The term $(1-\lambda)f_{\text{anc}}(x)$ in Eq.~ref{eq:SONAR_loss} acts as a static load. 

% On hard samples, this load is effectively zero (or noise), meaning the primary model only receives a fraction $\lambda$ of credit for its output. To achieve the full target $y$, it must exert $1/\lambda$ times the ``force'' (logit magnitude). 
% Crucially, when the auxiliary branch is removed at inference time, the model retains this amplified capacity. This \textbf{Compensatory Margin Expansion} pushes the decision boundary away from high-entropy regions, propelling the model out of the local optima where its historical self was trapped.

==> content/analysis.tex <==
% \section{ Why Can Weak Make Strong Stronger}
% \label{sec:theoretical_analysis}

% In this section, we provide two complementary theoretical views. First, we formalize why \textbf{joint logit mixing amplifies negative-token gradients}, yielding a principled advantage over standard SFT. Second, we retain the original margin-expansion analysis as a complementary lens on how compensatory pressure reshapes decision boundaries.
% \vspace{-10pt}
% \subsection{Why Joint Training Amplifies Hard-Negative Gradients}
% \label{sec:grad_amplification_main}
% Consider two models (Confuser/weak $m_{\mathrm{weak}}$, Learner/strong $m_{\mathrm{strong}}$) with logits $z_{\mathrm{weak}}, z_{\mathrm{strong}} \in \mathbb{R}^C$, and the mixed logits
% \begin{equation}
%     z_{\text{mix}} = (1-\lambda) z_{\mathrm{weak}} + \lambda z_{\mathrm{strong}}, \quad \lambda \in [0,1].
%     \label{eq:main_mix}
% \end{equation}
% Let $y$ denote the target index, $e_y$ the one-hot vector, and $p(z)=\text{Softmax}(z)$. The cross-entropy gradient on fused logits is
% \begin{equation}
%     g_{\text{mix}} = \nabla_{z_{\text{mix}}}\mathcal{L} = p(z_{\text{mix}}) - e_y,
%     \label{eq:main_grad_mix}
% \end{equation}
% while standard SFT on the Learner model gives $g_{\text{sft}} = p(z_{\mathrm{strong}}) - e_y$.

% \paragraph{Margins and hard negatives.}
% Define the target margin for any negative token $k \neq y$ as
% \begin{equation}
%     m_k(z) = z_y - z_k.
%     \label{eq:main_margin_def}
% \end{equation}
% The Confuser model encodes confusion, so we define the hard-negative set
% \begin{equation}
%     \mathcal{H} = \{ k \neq y : m_k(z_{\mathrm{weak}}) < m_k(z_{\mathrm{strong}}) \}.
%     \label{eq:main_hard_set}
% \end{equation}
% The mixed margin is a convex combination:
% \begin{equation}
%     m_k(z_{\text{mix}}) = (1-\lambda)m_k(z_{\mathrm{weak}}) + \lambda m_k(z_{\mathrm{strong}}).
%     \label{eq:main_margin_mix}
% \end{equation}

% \begin{theorem}[Total negative-mass increase under uniform margin shrinkage]
% If $m_k(z_{\mathrm{weak}}) \le m_k(z_{\mathrm{strong}})$ for all $k \neq y$, then
% \begin{align}
%     p(z_{\text{mix}})_y &\le p(z_{\mathrm{strong}})_y, \nonumber\\
%     \sum_{k \neq y} P(z_{\text{mix}})[k] &\ge \sum_{k \neq y} P(z_{\mathrm{strong}})[k].
%     \label{eq:main_total_neg_mass}
% \end{align}
% \end{theorem}
% \begin{proof}[Proof sketch]
% Using $p(z)_k/p(z)_y = \exp(-m_k(z))$, margin shrinkage implies $\exp(-m_k(z_{\text{mix}})) \ge \exp(-m_k(z_{\mathrm{strong}}))$ for all $k \neq y$, increasing the denominator of $p(z)_y$ and thus the total negative mass. A full proof is in Appendix~\ref{sec:appendix_grad_amp}.
% \end{proof}

% \begin{corollary}[Per-token amplification on hard negatives]
% For any $k \in \mathcal{H}$, the mixed negative gradient satisfies
% \begin{align}
%     P(z_{\text{mix}})[k] &\ge P(z_{\mathrm{strong}})[k] \quad \text{whenever} \nonumber\\
%     \frac{p(z_{\text{mix}})_y}{p(z_{\mathrm{strong}})_y}
%     &\ge \exp\!\left(-(1-\lambda)\Delta m_k\right),
%     \label{eq:main_amp_condition}
% \end{align}
% where $\Delta m_k = m_k(z_{\mathrm{strong}})-m_k(z_{\mathrm{weak}})>0$.
% \end{corollary}
% \begin{proof}[Proof sketch]
% Express $p_k$ via log-odds, substitute the mixed margin, and rearrange the ratio condition. See Appendix~\ref{sec:appendix_grad_amp} for the full derivation.
% \end{proof}

% \begin{proposition}[Logit updates emphasize negative suppression]
% Under joint training, for model $i \in \{1,2\}$ with scale $s_1=1-\lambda$, $s_2=\lambda$,
% \begin{align}
%     \Delta z_{i,k} &\approx -\eta s_i\, P(z_{\text{mix}})[k] \quad (k \neq y), \nonumber\\
%     \Delta z_{i,y} &\approx \eta s_i\, (1-p(z_{\text{mix}})_y).
%     \label{eq:main_update}
% \end{align}
% Thus any increase in $P(z_{\text{mix}})[k]$ directly amplifies suppression of hard negatives, while a decrease in $p(z_{\text{mix}})_y$ strengthens the upward push on the target logit.
% \end{proposition}
% \begin{proof}[Proof sketch]
% This follows from $\nabla_{z_i}\mathcal{L}=s_i(p(z_{\text{mix}})-e_y)$ and a first-order update $\Delta z_i \approx -\eta \nabla_{z_i}\mathcal{L}$. See Appendix~\ref{sec:appendix_grad_amp}.
% \end{proof}

% \paragraph{Interpretation.}
% These results formalize the key advantage over SFT: mixing logits redistributes probability mass toward hard negatives, which \emph{increases their gradients} and drives stronger suppression of incorrect tokens. This mechanism aligns with our empirical logit statistics (noise floor reduction and heavier tails) and provides a causal explanation for improved accuracy on hard tasks.

% \paragraph{Mechanistic interpretation (summary).}

% Beyond local gradients, joint training induces a three-stage dynamic: early gradient-share dominance of the Learner model (amplified by Confuser hard negatives), gradient shielding, and null-space drift. We include a formal analysis in Appendix~\ref{sec:appendix_joint_theory}; in short, the Confuser model exposes confusion regions early on, the Learner model takes the dominant update signal as it stabilizes, and mean-shift directions remain unconstrained. This interpretation complements the gradient-amplification view and explains the observed logit mean shifts.


% In this section, we also provide a complementary margin-expansion analysis under a linearized MSE regime, which offers an alternative perspective on how compensatory pressure reshapes decision boundaries.









\section{ Why Can Weak Make Strong Stronger}
\label{sec:theoretical_analysis}


In this section, we formalize the key advantage of weak-driven learning: 
\textbf{joint logit mixing with a weak agent amplifies informative gradients in saturated regions}, enabling continued optimization of strong agent beyond standard supervised fine-tuning.
We show that, by reintroducing probability mass to plausible but suppressed alternatives, joint training prevents gradient vanishing on non-target tokens and sustains effective learning pressure even after the strong model’s decision boundary has stabilized.

% In this section, we formalize why \textbf{joint logit mixing amplifies gradients in saturated regions}, yielding a principled advantage over standard SFT, and interpret the joint-training dynamics in terms of stage-wise behavior. We ground the analysis in the joint-training step defined in Eq.~\eqref{eq:logit_mix}--\eqref{eq:joint_sft_loss}.
\vspace{-10pt}
\subsection{Why Joint Training Amplifies Gradients in Saturated Regions}
\label{sec:grad_amplification_main}
Consider a weak agent $\mathcal{M}_{\mathrm{weak}}$ (initialized from a historical checkpoint and co-trained during joint training) and a strong agent $\mathcal{M}_{\mathrm{strong}}$ (current trainable agent) that, for a context $x$, produce logits $z_{\mathrm{weak}}(x), z_{\mathrm{strong}}(x) \in \mathbb{R}^{|\mathcal{V}|}$ over the vocabulary $\mathcal{V}$, and the mixed logits
\begin{equation}
    z_{\text{mix}}(x) = (1-\lambda) z_{\mathrm{weak}}(x) + \lambda z_{\mathrm{strong}}(x), \quad \lambda \in [0,1].
    \label{eq:main_mix}
\end{equation}
Operationally, $z_{\text{mix}}(x)$ is the fused logit map used for joint training, injecting the weak agent's uncertainty while preserving the strong agent's target direction.
Let $y$ denote the target index, $e_y$ the one-hot vector, and define $P_{\mathrm{mix}}(\cdot\mid x)=\mathrm{Softmax}(z_{\text{mix}}(x))$ and $P_{\mathrm{strong}}(\cdot\mid x)=\mathrm{Softmax}(z_{\mathrm{strong}}(x))$. More generally, for any logit map $z(x)$, let $P_z(\cdot\mid x)=\mathrm{Softmax}(z(x))$. The cross-entropy gradient on fused logits is
\begin{equation}
    g_{\text{mix}} = \nabla_{z_{\text{mix}}(x)}\mathcal{L} = P_{\mathrm{mix}}(\cdot\mid x) - e_y,
    \label{eq:main_grad_mix}
\end{equation}
For any negative token $k \neq y$, the gradient component is $g_{\text{mix}}[k] = P_{\mathrm{mix}}(k\mid x)$, so increasing negative probability mass directly increases the gradient magnitude on that token. Standard SFT on the strong agent gives $g_{\text{sft}} = P_{\mathrm{strong}}(\cdot\mid x) - e_y$ and can saturate when $P_{\mathrm{strong}}(k\mid x)$ is already small. \\
\textbf{Margins and hard negatives.}
Define the target margin for any negative token $k \neq y$ as
\begin{equation}
    m_k(z(x)) = z(x)[y] - z(x)[k].
    \label{eq:main_margin_def}
\end{equation}
The margin measures target-vs-distractor separation: smaller margins mean higher confusion. We define the hard-negative set
\begin{equation}
    \mathcal{H} = \{ k \neq y : m_k(z_{\mathrm{weak}}(x)) < m_k(z_{\mathrm{strong}}(x)) \}.
    \label{eq:main_hard_set}
\end{equation}
These are tokens where the weak agent is less separated than the strong agent, i.e., the weak agent highlights unresolved boundaries. The mixed margin is a convex combination:
\begin{equation}
    m_k(z_{\text{mix}}(x)) = (1-\lambda)m_k(z_{\mathrm{weak}}(x)) + \lambda m_k(z_{\mathrm{strong}}(x)).
    \label{eq:main_margin_mix}
\end{equation}
Thus mixing shrinks margins toward the weak agent on $\mathcal{H}$, raising the relative probability of hard negatives.

\begin{theorem}[Total negative-mass increase under uniform margin shrinkage]
If $m_k(z_{\mathrm{weak}}(x)) \le m_k(z_{\mathrm{strong}}(x))$ for all $k \neq y$, then
\begin{align}
    P_{\mathrm{mix}}(y\mid x) &\le P_{\mathrm{strong}}(y\mid x), \nonumber\\
    \sum_{k \neq y} P_{\mathrm{mix}}(k\mid x) &\ge \sum_{k \neq y} P_{\mathrm{strong}}(k\mid x).
    \label{eq:main_total_neg_mass}
\end{align}
\end{theorem}
The theorem shows that, when the weak agent is uniformly more uncertain than the strong agent, joint logit mixing necessarily shifts probability mass from the target to negative tokens.
As a consequence, gradient magnitude on negative classes is amplified, preventing vanishing gradients in saturated regions.
This mechanism explains why weak-driven learning enables continued refinement of the strong agent’s decision boundary even after standard supervised fine-tuning has converged.
A complete proof is provided in Appendix~\ref{sec:appendix_grad_amp}.

% Operationally, if the weak agent is uniformly more confused than the strong agent, mixing shifts probability mass toward negatives, preventing gradients in saturated regions from vanishing. A full proof is in Appendix~\ref{sec:appendix_grad_amp}.

% \begin{proof}[Proof sketch]
% Using $P_z(k\mid x)/P_z(y\mid x) = \exp(-m_k(z(x)))$ for any logit map $z(x)$, margin shrinkage implies $\exp(-m_k(z_{\text{mix}}(x))) \ge \exp(-m_k(z_{\mathrm{strong}}(x)))$ for all $k \neq y$, increasing the denominator of $P_{\mathrm{mix}}(y\mid x)$ and thus the total negative mass. A full proof is in Appendix~\ref{sec:appendix_grad_amp}.
% \end{proof}


 
\begin{corollary}[Per-token amplification on hard negatives]
For any $k \in \mathcal{H}$, the mixed negative gradient satisfies
\begin{align}
    P_{\mathrm{mix}}(k\mid x) &\ge P_{\mathrm{strong}}(k\mid x) \quad \text{whenever} \nonumber\\
    \frac{P_{\mathrm{mix}}(y\mid x)}{P_{\mathrm{strong}}(y\mid x)}
    &\ge \exp\!\left(-(1-\lambda)\Delta m_k\right),
    \label{eq:main_amp_condition}
\end{align}
where $\Delta m_k = m_k(z_{\mathrm{strong}}(x))-m_k(z_{\mathrm{weak}}(x))>0$.
\end{corollary}

This corollary provides a token-level characterization of gradient amplification:
for hard negatives, joint logit mixing increases their assigned probability—and thus their gradient magnitude, under mild and explicit conditions on the relative target probabilities.


% This gives a token-level criterion: for hard negatives, the mixed distribution raises their probability (and gradient) under mild conditions on the target probability ratio.

% \begin{proof}[Proof sketch]
% Express $p_k$ via log-odds, substitute the mixed margin, and rearrange the ratio condition. See Appendix~\ref{sec:appendix_grad_amp} for the full derivation.
% \end{proof}

\begin{proposition}[Logit updates on negative and target tokens]
Under joint training, for agent $i \in \{\mathrm{weak},\mathrm{strong}\}$ with scale $s_{\mathrm{weak}}=1-\lambda$, $s_{\mathrm{strong}}=\lambda$,
\begin{align}
    \Delta z_{i,k} &\approx -\eta s_i\, P_{\mathrm{mix}}(k\mid x) \quad (k \neq y), \nonumber\\
    \Delta z_{i,y} &\approx \eta s_i\, (1-P_{\mathrm{mix}}(y\mid x)).
    \label{eq:main_update}
\end{align}
Thus any increase in $P_{\mathrm{mix}}(k\mid x)$ directly amplifies suppression of hard negatives, while a decrease in $P_{\mathrm{mix}}(y\mid x)$ strengthens the upward push on the target logit.
\end{proposition}
The proposition shows that any increase in the mixed probability
$P_{\mathrm{mix}}(k \mid x)$ directly amplifies the suppressive update on
non-target tokens, while a corresponding decrease in
$P_{\mathrm{mix}}(y \mid x)$ strengthens the upward update on the target
logit.
These dynamics are consistent with the empirical reduction of the
non-target logit mean observed in our logit statistics.




\vspace{-0.1cm}
\begin{tcolorbox}[
    colback=blue!2,
    colframe=blue!40!black,
    boxrule=0.6pt,
    arc=2pt,
    left=6pt,
    right=6pt,
    top=0pt,
    bottom=0pt
]
\textbf{Summary (Why Weak-Driven Learning Works):}
These theoretical results formalize the key advantage of weak-driven learning over standard SFT.
By redistributing probability mass toward hard negatives in saturated regions, joint logit mixing with a weak agent increases gradient magnitudes for the strong agent that would otherwise vanish under SFT.
While the dominant effect arises from amplified suppression of non-target tokens, the concurrent reduction in target probability further strengthens the positive update on the correct class.
Together, these effects alleviate optimization saturation and enable the strong agent to continue refining its decision boundary beyond the convergence point of conventional supervised fine-tuning.
\end{tcolorbox}


% These results formalize the key advantage over SFT: mixing logits redistributes probability mass in saturated regions, \emph{increasing gradients that would otherwise vanish}. The dominant effect is on non-target tokens (hard negatives), while a decrease in $P_{\mathrm{mix}}(y\mid x)$ strengthens the upward update on the target.
% Informally, this extra gradient signal relative to SFT reduces saturation and can help optimization move past local minima during training.


% \begin{proof}[Proof sketch]
% This follows from $\nabla_{z_i}\mathcal{L}=s_i(P_{\mathrm{mix}}(\cdot\mid x)-e_y)$ and a first-order update $\Delta z_i \approx -\eta \nabla_{z_i}\mathcal{L}$. See Appendix~\ref{sec:appendix_grad_amp}.
% \end{proof}

Mechanistic interpretation (three stages) of weak-driven learning:

\textbf{Stage I: saturated-region amplification.} Early in joint training, the weak agent is more confused on many non-target tokens, so mixing increases total negative mass (Appendix~\ref{sec:appendix_grad_amp}, Eq.~\eqref{eq:appendix_total_neg_mass}); $g_{\text{mix}}$ is biased toward hard negatives, and the strong agent dominates the effective update (Appendix~\ref{sec:appendix_joint_theory}, Eq.~\eqref{eq:appendix_dominance}).\\
\textbf{Stage II: gradient shielding.} As the strong agent becomes confident, the Softmax Hessian collapses (Appendix~\ref{sec:appendix_joint_theory}, Eq.~\eqref{eq:appendix_hessian_collapse}) and the cross-Hessian between agents vanishes (Eq.~\eqref{eq:appendix_cross_hessian}). The weak agent then receives little curvature information, so its influence on training diminishes even though it still provides the fused logits.\\
\textbf{Stage III: null-space drift.} Because Softmax is invariant to global logit shifts (Eq.~\eqref{eq:appendix_softmax_shift}), the loss is flat along the mean direction. When gradients are small, stochastic updates can drift in this null space, producing the observed mean-logit drift without changing centered sharpness (Appendix~\ref{sec:appendix_joint_theory}).






==> table/grpo_results.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Impact of Initialization on Post-Training GRPO.} We compare the performance of Group Relative Policy Optimization (GRPO) when initialized from a standard SFT checkpoint versus a \textsc{SCORE} checkpoint. All experiments use Qwen3-4B-Base. \textsc{SCORE} provides a superior ``launchpad,'' enabling GRPO to reach significantly higher performance ceilings.}
    \label{tab:grpo_results}
    
    % 定义浅灰色用于高亮
    \definecolor{mygray}{gray}{0.92}
    \setlength{\tabcolsep}{5pt}
    
    \begin{small}
    \begin{sc}
        \begin{tabular}{l l | c c >{\columncolor{mygray}}c}
            \toprule
            \textbf{METHOD} & \textbf{Stage} & \textbf{MATH500} & \textbf{AIME2025} & \textbf{Avg.} \\
            \midrule
            % Group 1: Standard SFT route
            \multirow{2}{*}{SFT} 
              & None & 66.1 & 12.2 & 39.1 \\
              & + GRPO & 85.8 & 20.0 & 52.9 \\
            \midrule
            % Group 2: SCORE route
            \multirow{2}{*}{\textbf{SCORE}} 
              & None & 72.1 & 20.0 & 46.0 \\
              & \textbf{+ GRPO} & \textbf{85.0} & \textbf{26.7} & \textbf{55.9} \\
            \midrule
            \multicolumn{2}{c|}{\textit{Net Gain via SCORE-Init}} & \textcolor{blue}{\textbf{-0.8}} & \textcolor{blue}{\textbf{6.7}} & \textcolor{blue}{\textbf{3.0}} \\
            \bottomrule
        \end{tabular}
    \end{sc}
    \end{small}
\end{table}


==> table/main_results_copy.tex <==
\begin{table*}[t!]
    \centering
    \caption{\textbf{Main Results on Qwen3-4B-Base and Qwen3-8B-Base.} We benchmark \textsc{SCORE} against standard SFT and noise-injected baselines (NEFTune) across 7 math datasets and 2 code benchmarks. All models are fine-tuned for a total of 2 epochs. ``GS'' denotes Gaussian Noise injection. \textbf{Bold} indicates the best performance, and \underline{underline} denotes the second best.}
    \label{tab:main_results}
    % 使用 resizebox 确保表格宽度自适应页面，字体不用手动设为 tiny
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l|c c c c c c c c|c c c}
        \toprule
        \multirow{2}{*}{\textbf{Methods}} & \multicolumn{8}{c}{\textbf{Math}} &  \multicolumn{3}{c}{\textbf{Code}} \\
        \cmidrule(l){2-9}\cmidrule(l){10-12}
         &\textbf{AIME2025} & \textbf{MATH500} & \textbf{AMC23} & \textbf{AQUA} & \textbf{GSM8K} & \textbf{MAWPS} & \textbf{SVAMP}& Avg. & \textbf{HumanEval} & \textbf{MBPP} & Avg. \\
        \midrule
        \multicolumn{12}{c}{\textit{Qwen3-4B-Base as base model.}} \\
        \midrule
         % SFT & 1 & 10.7 & 64.9 && 56.3 & 82.3 & 90.1 & 83.3 & 64.6 & 68.5 & 57.7 & \\
         SFT& 12.2 & 66.1 & \underline{47.7} & \underline{61.8} & 83.9 & 91.3 & 85.5 & 64.1 & 68.5 & \underline{57.7} & 63.1\\
         % SFT & 3 & 12.0 & 67.4 & 54.7 & 85.1 & 95.4 & 87.7 & 67.1 \\
         SFT + GS & 12.2 & 63.1 & 40.0 & 55.1 & 82.9 & 90.9 & 84.1 & 61.2 & 71.3 & 54.6 & 63.0\\
         NEFTune & \underline{16.7} & \underline{68.2} & 43.3 & 58.9 & \underline{86.7} & \underline{93.8} & \underline{87.7} & \underline{65.0} & \underline{74.2} & 55.1 & \underline{64.7} \\
         % SCORE-stage1 & 2 & \underline{13.3} & \underline{69.4} & \underline{62.0} & \underline{86.2} & \underline{93.7} & \underline{87.3} & \underline{68.7} & 74.4 & 59.2 & \\
         \textbf{\textsc{SCORE}} & \textbf{20.0} & \textbf{71.3} & \textbf{50.0} & \textbf{67.6} & \textbf{88.5} & \textbf{96.2} & \textbf{90.3} & \textbf{69.1} & \textbf{74.4} & \textbf{59.2} & \textbf{66.8}\\
         % \textbf{\textsc{SCORE}} & 3 & \textbf{20.0} & \textbf{73.3} & \textbf{71.8} & \textbf{91.4} & \textbf{95.7} & \textbf{92.6} & \textbf{74.6} & \textbf{76.4} & \textbf{59.8} \\
         % SCORE & 4 & \textbf{23.3} & \textbf{73.7} & \textbf{74.3} & \textbf{90.2} & \textbf{97.9} & \textbf{93.6} & \textbf{75.5} \\
         % SCORE & 5 & 10.0 & 51.8 & 66.5 & 91.2 & 97.5 & 93.9 & 67.1 \\
         % \cmidrule{2-9}
        % \textbf{\textsc{SCORE} (Ours)} & \textbf{79.5} & \underline{36.6} & \textbf{71.8} & \underline{43.8} & \textbf{73.2} & \underline{66.1} & \textbf{62.0} \\
        \midrule
        \multicolumn{12}{c}{\textit{Qwen3-8B-Base as base model.}} \\
        \midrule
         % SFT & 1 & 10.3 & 70.3 & 61.8 & 86.1 & 94.3 & 86.3 & 68.2 & 76.2 & 64.0 \\
         SFT & \underline{15.6} & 72.1 & \underline{45.0} & 63.0 & 87.5 & 95.1 & 88.6 & 66.7 & 78.3 & 64.0 & 71.2\\
         SFT+GS & 10.0 & 71.5 & 48.3 & 66.9 & 89.9 & 96.4 & 91.2 & 67.7 & 79.7 & 61.0 & 70.4\\
         NEFTune & \underline{15.6} & \underline{73.7} & 40.0 & \underline{71.3} & \underline{90.3} & \underline{97.3} & \underline{91.5} & \underline{68.5} & \underline{80.5} & \underline{64.3} & \underline{72.4} \\
         % SFT & 3 & 12.0 & 73.7 & 61.3 & 89.2 & 95.7 & 90.2 & 70.4\\
         % SCORE & 2 & \underline{17.8} & \underline{75.4} & \underline{68.0} & \underline{90.6} & \underline{95.8} & \underline{89.8} &  \underline{72.9} & 80.3 & 70.0\\
         \textbf{\textsc{SCORE}} & \textbf{20.0} & \textbf{75.4} & \textbf{52.5} & \textbf{77.3} & \textbf{92.5} & \textbf{97.8} & \textbf{94.0} &  \textbf{72.9} & \textbf{83.9} & \textbf{71.3} & \textbf{77.6}\\
        \bottomrule
    \end{tabular}
    }
    
\end{table*}

==> table/sensitive_of_lambda.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Post-hoc sensitivity analysis of mixing coefficient $\lambda$.} We report pass@1 accuracy (\%) under greedy decoding on Qwen3-4B-Base across varying $\lambda$ values. This diagnostic sweep is not used to select the headline models in Table~\ref{tab:main_results}; those runs use the fixed default $\lambda=0.5$.}
    \label{tab:sensitive_of_lambda}
    
    % 稍微调整列间距
    \setlength{\tabcolsep}{8pt}
    
    \begin{small}
    \begin{sc}
        \begin{tabular}{l ccccc}
            \toprule
            \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{5}{c}{\textbf{Mixing Coefficient} $\lambda$} \\
            \cmidrule(l){2-6}
             & 0.46 & \textbf{0.48} & 0.5 & 0.52 & 0.54 \\
            \midrule
            % 这里填入您实际或预估的数据，呈现中间高两边低的趋势
            AMIE    & 16.7 & \textbf{20.0} & 17.8 & 21.1 &  16.7\\
            MATH500 & 73.1 & \textbf{73.3} & 71.1 & 70.7 &  74.0\\
            AQUA    & 72.4 & \textbf{71.8} & 73.9 & 71.0 &  71.3\\
            GSM8K   & 91.0 & \textbf{91.4} & 89.0 & 91.2 &  91.4\\
            MAWPS   & 97.8 & \textbf{98.0} & 95.7 & 96.5 &  97.2\\
            SVAMP   & 93.5 & \textbf{92.9} & 92.6 & 92.4 & 93.5 \\
            \midrule
            \textit{Avg.} & 74.1 & \textbf{74.6} & 73.4 & 73.8 & 74.0 \\
            \bottomrule
        \end{tabular}
    \end{sc}
    \end{small}
    \vskip -0.1in
\end{table}

